The more legs the merrier: A new composition for symmetric (multi-)lenses

Lenses are a category theoretic construct and are used in a wide variety of applications. Symmetric lenses compose to, of course, form new symmetric lenses. Symmetric lenses are usually represented as spans of asymmetric lenses. In many applications, the fact that a symmetric lens might also be represented as a cospan of asymmetric lenses is important, especially for implementation purposes. However, the composition of symmetric lenses does not preserve the property that the lenses can be represented by cospans -- two such symmetric lenses may (and frequently do) compose to form a symmetric lens which cannot be represented as a cospan of asymmetric lenses. Thus preserving the factorisation to show how cospans of asymmetric lenses might be used in implementations becomes important. In 2018, the first work on multilenses was begun. Multilenses can be represented as multi-spans of asymmetric lenses (often called 'wide spans', these are spans with an arbitrary finite number of legs). In this paper we analyse a small but realistic example of a supply chain in which the cospan representations would be 'composed away' by ordinary symmetric lens composition, and introduce a new kind of composition which we call 'fusion' in which two ordinary symmetric lenses (spans with two legs) fuse to form a multilens with three legs preserving the cospan representations, and more generally, two symmetric multilenses, spans with say m and n legs, fuse to form a symmetric multilens with m+n-1 legs, again preserving cospan representations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{92}
\providecommand{\publicationstatus}{David I. Spivak and Jamie Vicary (Eds.):\\
Applied Category Theory 2020 (ACT2020)\\
EPTCS 333, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.333.7}{10.4204/EPTCS.333.7}}

